YTrace: End-to-end Performance Diagnosis in Large Cloud and Content Providers

Content providers build serving stacks to deliver content to users. An important goal of a content provider is to ensure good user experience, since user experience has an impact on revenue. In this paper, we describe a system at Yahoo called YTrace that diagnoses bad user experience in near real time. We present the different components of YTrace for end-to-end multi-layer diagnosis (instrumentation, methods and backend system), and the system architecture for delivering diagnosis in near real time across all user sessions at Yahoo. YTrace diagnoses problems across service and network layers in the end-to-end path spanning user host, Internet, CDN and the datacenters, and has three diagnosis goals: detection, localization and root cause analysis (including cascading problems) of performance problems in user sessions with the cloud. The key component of the methods in YTrace is capturing and discovering causality, which we design based on a mix of instrumentation API, domain knowledge and blackbox methods. We show three case studies from production that span a large-scale distributed storage system, a datacenter-wide network, and an end-to-end video serving stack at Yahoo. We end by listing a number of open directions for performance diagnosis in cloud and content providers.

==> Makefile <==
REPORT=paper
LATEX=latex
BIBTEX=bibtex --min-crossrefs=1000
REF1=ref

TEX = $(wildcard *.tex)
CLS = $(wildcard *.cls)
SRCS = $(TEX)
REFS=$(REF1).bib

all: pdf
#.tex.dvi:
#       $(LATEX) $*.tex

#$(REPORT).dvi: figures $(SRCS) $(CLS) paper.bib
$(REPORT).dvi: $(SRCS) $(CLS) $(REF1).bib
	$(LATEX) $(REPORT)
	$(BIBTEX) $(REPORT)
	perl -pi -e "s/%\s+//" $(REPORT).bbl
	$(LATEX) $(REPORT)
	$(LATEX) $(REPORT)

#$(REPORT).ps: $(REPORT).dvi figures
$(REPORT).ps: $(REPORT).dvi 
	dvips -Pcmz -t letter $(REPORT).dvi -o $(REPORT).ps
#	dvips -Ppdf -G0 -t letter $(REPORT).dvi -o $(REPORT).ps



#not relevant here
#figures:
#	cd figures; make


view: $(REPORT).dvi
	xdvi $(REPORT).dvi

print: $(REPORT).dvi
	dvips $(REPORT).dvi

pdf: $(REPORT).ps
	ps2pdf14 $< $(REPORT).pdf

printer: $(REPORT).ps
	lpr $(REPORT).ps

tidy:
	rm -f *.dvi *.aux *.log *.blg *.bbl

clean:
	rm -f *~ *.dvi *.aux *.log *.blg *.bbl $(REPORT).ps $(REPORT).pdf $(PROPOSAL).ps $(PROPOSAL).pdf $(FIRSTDRAFT).ps $(FIRSTDRAFT).pdf


